Hybrid Neural Fusion for Full-frame Video Stabilization

Existing video stabilization methods often generate visible distortion or require aggressive cropping of frame boundaries, resulting in smaller field of views. In this work, we present a frame synthesis algorithm to achieve full-frame video stabilization. We first estimate dense warp fields from neighboring frames and then synthesize the stabilized frame by fusing the warped contents. Our core technical novelty lies in the learning-based hybrid-space fusion that alleviates artifacts caused by optical flow inaccuracy and fast-moving objects. We validate the effectiveness of our method on the NUS, selfie, and DeepStab video datasets. Extensive experiment results demonstrate the merits of our approach over prior video stabilization methods.

==> 6_limitation.tex <==
\section{Limitations}
\label{sec:limitation}

Video stabilization for videos in unconstrained scenarios remains challenging. 
Here we discuss several limitations of our approach. 
We refer to the readers to our supplementary material for video results.

\topic{Wobble.} 
When the camera or object motion is too rapid, we observe that the stabilized frame exhibit \emph{rolling shutter wobble} (\figref{failure_cases}(a)). 
Integrating rolling shutter rectification into our approach can potentially alleviate such an issue.

\topic{Visible seams.} 
As our method fuse multiple frames to re-render a stabilized frame, our results may contain visible seams, particularly when there are large lighting variations caused by camera white‐balancing and exposure corrections (\figref{failure_cases}(b)).

\topic{Temporal flicker and distortion.} 
Our method builds upon an existing motion smoothing method~\cite{yu2020learning} to obtained stabilized frames. 
However, the method~\cite{yu2020learning} may produce temporally flickering results due to large non-rigid occlusion and inconstant foreground/background motion (e.g., selfie videos). 
In such cases, due to the dependency of motion inpainting, our method also suffers from undesired temporal flicker and distortion (\figref{failure_cases}(c)).

\topic{Speed.} Our work aims for offline application. 
Currently, our method runs slowly (about 10 seconds/frame) compared to many existing methods.
Speeding up the runtime is important future work.



\input{figs/fig_failure_cases}


==> figs/fig_failure_cases.tex <==
\begin{figure*}[h!]
\centering
\renewcommand{\tabcolsep}{2pt} %
\renewcommand{\arraystretch}{1} %
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc}
\includegraphics[width=0.35\textwidth, height=0.2\textwidth]{figures/failure_cases/wobble.jpg} & 
\includegraphics[width=0.35\textwidth, height=0.2\textwidth]{figures/failure_cases/light.jpg} & 
\includegraphics[width=0.35\textwidth, height=0.2\textwidth]{figures/failure_cases/flow_fail2.jpg} \\
(a) Wobble & (b) Visible seams & (c) Temporal flicker and distortion \\
\end{tabular}
}
\caption{
\textbf{Limitations.}
(a) Our method does not correct rolling shutter and thus may suffer wobble artifacts.
(b) Our fusion approach is not capable of compensating large photometric variations across frames, resulting in visible seams.
(c) Existing smoothing approach \cite{yu2020learning} may introduce distortion, particularly when videos contain non-rigid large occlusion (such as selfie videos). As our method depends on the flow produced by \cite{yu2020learning} for stabilizing the video, we cannot correct such errors. 
}
\label{fig:failure_cases}
\end{figure*}

